Generalization Bounds for Gradient Methods via Discrete and Continuous Prior

Proving algorithm-dependent generalization error bounds for gradient-type optimization methods has attracted significant attention recently in learning theory. However, most existing trajectory-based analyses require either restrictive assumptions on the learning rate (e.g., fast decreasing learning rate), or continuous injected noise (such as the Gaussian noise in Langevin dynamics). In this paper, we introduce a new discrete data-dependent prior to the PAC-Bayesian framework, and prove a high probability generalization bound of order $O(\frac{1}{n}\cdot \sum_{t=1}^T(\gamma_t/\varepsilon_t)^2\left\|{\mathbf{g}_t}\right\|^2)$ for Floored GD (i.e. a version of gradient descent with precision level $\varepsilon_t$), where $n$ is the number of training samples, $\gamma_t$ is the learning rate at step $t$, $\mathbf{g}_t$ is roughly the difference of the gradient computed using all samples and that using only prior samples. $\left\|{\mathbf{g}_t}\right\|$ is upper bounded by and and typical much smaller than the gradient norm $\left\|{\nabla f(W_t)}\right\|$. We remark that our bound holds for nonconvex and nonsmooth scenarios. Moreover, our theoretical results provide numerically favorable upper bounds of testing errors (e.g., $0.037$ on MNIST). Using a similar technique, we can also obtain new generalization bounds for certain variants of SGD. Furthermore, we study the generalization bounds for gradient Langevin Dynamics (GLD). Using the same framework with a carefully constructed continuous prior, we show a new high probability generalization bound of order $O(\frac{1}{n} + \frac{L^2}{n^2}\sum_{t=1}^T(\gamma_t/\sigma_t)^2)$ for GLD. The new $1/n^2$ rate is due to the concentration of the difference between the gradient of training samples and that of the prior.

==> _results.tex <==


This paper attempts to provide a way to circumvent these problems, and to provide a possible idea to obtain a tighter generalization error bound (e.g., $O(1/n + T/n^2)$). The framework we use in this paper is Catoni's PAC-Bayesian~\citep{catoni2007pac}. In particular, we use its data-dependent version (see Theorem~\ref{thm:data-pac} for details). Roughly speaking, the testing error is bounded by the following quantity with high probability over $S\sim \D^n$ and random subset $J\subset [n]$ with size $m$:
\[(\forall Q)\quad c_0\risk(Q, S_{[n]\backslash J}) + c_1\cdot \frac{\Theta(1) + \KL{Q}{P(S_J)}}{n-m},\]
where $Q$ is usually chosen to be the distribution of trained model, and $P(S_J)$ can be any prior distribution only depends on $S_J$ (a subset of $S$). The key is to choose a proper prior. A straightforward idea is to make the prior $P(S_J)$ directly imitate $Q_S$. For example, if $Q_S$ is obtained by running an algorithm on $S$, then for prior $P(S_J)$ we also run the \emph{same algorithm} on $S_J$. This idea is used in \citet{xxx} for proving generalization bound for noisy gradient methods such as SGLD.  However, this approach suffers from the ``infinite-KL'' problem when applied to discrete GD/SGD. Let's consider a one-step GD. Then the posterior $Q_S$ is a point mass at $W_1 = w_0 - \g f(w_0,S)$ while the prior $P(S_J)$ is a point mass at $W'_1 = w_0 \g f(w_0, S_J)$. Note that the two gradients are always different. By the definition of KL-divergence, we have $\KL{W_1}{W'_1} = 1\cdot \log (1/0) = \infty$. Therefore, if we want to deal with discrete algorithm such as gradient descent, we can't simply make $P(S_J)$ run the same algorithm as $Q_S$. In this paper, we propose a new way to construct data-dependent prior $P(S_J)$ that can avoid this problem. Moreover, we provide another idea to improve the PAC-Bayesian bound by noticing the concentration property of prior gradient.


\paragraph{Floored Gradient Descent (FGD).}
Let us consider a variant of gradient descent called Floored Gradient Descent (FGD).
First, we decompose $\g f(W_t, S)= \g f(W_t, S_J) + (\g f(W_t, S)-\g f(W_t, S_J))$
where $J\subset S$.
We round the second term to an integral multiply of $\eps$ 
and update the parameter as follows (see Algorithm~\ref{alg:fgd} for details):
\begin{align*}\label{eq:fgd}
  W_{t+1} \gets W_{t} - \gamma_t \g f(W_t, S_J) - \eps \cdot \floor\left(\frac{\gamma_t \g f(W_t,S) - \gamma_t \g f(W_t, S_J)}{\eps}\right), \tag{FGD}
\end{align*}
where $W_0 = w_0$ is the initial parameter, $\floor(x)$ equals to $\lfloor x\rfloor$ for $x > 0$ and $-\lfloor -x\rfloor$ otherwise. Notice that the FGD becomes GD as $\eps\to 0$ or we ignore the floor operation. Hence, FGD can be thought as a low precision version of GD (with precision level $\epsilon$).
By the definition of FGD, we can see that it is a deterministic algorithm. 
SAY SOMETHING FGD WORKS VERY CLOSE TO GD. ANY REFERENCE?

\paragraph{Discrete prior.} 
Note that the data-dependent PAC-Bayesian bound is still valid even when $W_T$ is depending on the prior. Our goal is to construct a discrete prior $P(S_J)$ such that $\KL{W_T}{P(S_J)}$ is small. 
Now let's construct the prior $P(S_J)$ step by step. At each step $t$, the first part of FGD gradient $\gamma_t \g f(W_t, S_J)$ is visible. Thus we only need to predict the difference term $a_t = \floor((\gamma_t \g f(W_t, S) - \gamma_t \g f(W_t,S_J))/\eps) \in \mathbb{Z}$. Intuitively, when $|J|$ is sufficiently large (i.e. $n/2$), the difference $\alpha_t$ should be very close to $0$. Based on this 
conjecture, we assign most of the probability to grid points close to $0$. The detailed construction is presented in Algorithm~\ref{alg:prior-fgd}. Under this construction, we are able to achieve a $O(\gamma_t^2\norm{\g f(W_t,S)- \g f(W_t,S_J)}^2/\eps^2)$ KL bound for each step. Then, we use the chain-rule of KL divergence to bound $\KL{W_T}{P(S_J)}$ by the sum of each step's KL (see Theorem~\ref{thm:fgd}).

\paragraph{Concentration for prior gradient.}
Intuitively, the difference $\norm{\g f(W_t,S) - \g f(W_t, S_J)}^2$ should be $O(1/m)$ (see Figure~\ref{fig:mgrad}), where $m=|J|$. Unfortunately, $W_t$ and $J$ are not independent. It is not very easy to prove a concentration inequality for FGD. However, when it comes to the algorithm that is independent of $J$ such as Langevin Dynamics (LD) and Stochastic Gradient Langevin Dynamics (SGLD), we can prove this concentration (Lemma~\ref{lem:gld-grad-con}) by a modified McDiarmid inequality (Lemma~\ref{lem:new-mcd}). Then we are able to obtain an $O(\frac{T}{m(n-m)})$ generalization bound (see Theorem~\ref{thm:gld-bound}).

Our results can be divided into two parts. The first part is the generalization bound for deterministic algorithm, the second part is the new generalization bounds for stochastic gradient methods such as GLD, SGLD, and CLD.
\paragraph{Generalization for FGD and FSGD.} We first prove algorithm-dependent generalization bound (more precisely, a test error bound) for FGD (Algorithm~\ref{alg:fgd}) and FSGD (Algorithm~\ref{alg:fsgd}). FGD and FSGD are close variants of GD and SGD, respectively. Formally, we show that w.p. $\geq 1-\delta$ over $S\sim \D^n$ and random indices $J$ of size $n/2$, the output $W_T$ of FGD satisfies:
\begin{align*}
\risk(W_T,\D) &\leq 1.59 \cdot \risk(W_T,S_I) + 3.17 \cdot \frac{\ln(1/\delta) + 3}{n}\\
&+\frac{3.17 \cdot\ln(dT)}{n\eps^2}\sum_{t=1}^T\left( \gamma_t^2\norm{\g f(W_{t-1},S)-\g f(W_{t-1},S_J)}_2^2\right).
\end{align*}
Compared to other generalization bounds~\citep{xxx} for SGD or GD, our analysis enjoys the following advantages:
\begin{enumerate}
    \item We don't need to add a Gaussian noise on the trained model or each step gradient. We directly study the generalization of the deterministic algorithm. 
    \item Our bound holds for the non-convex and non-smooth scenario. Moreover, we don't require the loss to be Lipschitz.
    \item In the experiment (Figure~\ref{fig:fgd-mnist-exp}) for MNIST + CNN ($\#$ param = 1.4M), our bound provides a $\mathbf{5.48\%}$ high probability bound for the testing error which is better than the $46\%$ bound reported in \citet{ZhouVAAO19} and the $16.1\%$ bound reported in \citet{dziugaite2017computing}.
\end{enumerate}

\paragraph{Generalization for noisy gradient methods.} We first prove concentration properties for the prior gradient (Lemma~\ref{lem:gld-grad-con} and~\ref{lem:cld-grad-con}). Then we are able to prove a tighter generalization bounds for 

==> _rgd.tex <==
\subsection{Rounded Gradient Descent}
First, we need to define the ``rounding'' procedure.
\begin{definition}[Rounding] For any $x \in \R$, we define 
$\round(x) \gets \lfloor x\rfloor + R,$
where $R$ is a fair coin such that $\Pr[R=1] = \Pr[R=0] = 1/2$.
The definition can be adapted to $X\in \R^d$ by setting
\[\round(X) = (\round(X_1),...,\round(X_d))^\top.\]
\end{definition}
Now we are ready to define our Rounded Gradient Descent (RGD) algorithm. As presented in Algorithm~\ref{alg:rgd}, the only difference to GD is that we round the gradient at each step. 
\begin{algorithm}
\KwIn{Training dataset $S=(z_1,..,z_n)$.}
\KwResult{Parameter $W_T\in \R^d$.}
\caption{Rounded Gradient Descent\label{alg:rgd}}
Initialize $W_0\sim \mu_0$\;
\For {$t:1\to T$} {
    $W_t \gets W_{t-1} - \eps\cdot \round(\frac{\gamma_t\g f(W_{t-1},S)}{\eps})$\;
}
\end{algorithm}
\begin{algorithm}
\KwIn{Prior dataset $S_J$.}
\KwResult{Parameter $W'_T\in \R^d$.}
\caption{Prior for RGD\label{alg:prior-rgd}}
Initialize $W'_0\sim \mu_0$\;
\For {$t:1\to T$} {
    $W'_t \gets W'_{t-1} - \eps\cdot \round(\frac{\gamma_t\g f(W'_{t-1},S_J)}{\eps}) + \xi_t$\;
    \tcp{$\xi_t$ is a discrete random variable such that} \tcp{$\Pr[\xi_t = (a_1,...,a_d)^\top] = \left(\sum_{i=-\infty}^{\infty}p^{i^2}\right)^{-d}\exp\left(-\sum_{k=1}^d \ln(1/p) a_k^2\right),$}
    \tcp{where $(a_k)_{k\in[d]} \in \mathbb{Z}^d$ are integers and $p\in(0,\frac{1}{3})$.}
}
\end{algorithm}
The following theorem depicts the generalization property of RGD.
\begin{theorem}\label{thm:rgd}
Suppose $J$ is a random sequence consisting of $m$ indices uniformly sampled from $[n]$ without replacement. Then for any $\delta \in (0,1),\eps \in (0, 1)$ and $p \in (0, \frac{1}{3})$, the RGD (Algorithm~\ref{alg:rgd}) satisfies the following generalization bound w.p. at least $1-\delta$ over $S\sim \D^n$ and $J$:
\begin{align*}
\risk(Q,\D) &\leq \eta C_{\eta}\risk(Q,S_I) + C_{\eta}\cdot \frac{\ln(1/\delta) + 3}{n-m}\\
&+\frac{C_{\eta}\ln(dT)}{(n-m)\eps^2}\sum_{t=1}^T\E\left[ \gamma_t^2\norm{\g f(W_{t-1},S)-\g f(W_{t-1},S_J)}_2^2\right],
\end{align*}
where $d$ is the dimension of parameter space, $Q$ is the distribution of $W_T$, $I = [n]\backslash \set(J)$ are indices that are not in $J$, and $C_{\eta}:=\frac{1}{1-e^{-\eta}}$ is a constant.
\end{theorem}
\begin{proof}
Similar to the proof of Theorem~\ref{thm:fgd}, we first construct a data-dependent prior in Algorithm~\ref{alg:prior-rgd}. Applying the chain rule of KL-divergence, we have
\begin{equation}\label{eq:rgd}
\begin{split}
\KL{Q}{P(S_J)}&:= \KL{W_T}{W'_T}\\
&\leq \sum_{t=1}^T\E_{w\sim W_{t-1}}[\KL{W_t|W_{t-1}=w}{W'_t|W'_{t-1}=w}].
\end{split}
\end{equation}
For any fixed $w \in \R^d$, let $X=W_t|W_{t-1}=w$ and $X'=W'_t|W'_{t-1}=w$. Recall that our round procedure is stochastic. We construct two random sequences $(R, X_t)$ and $(R', X'_t)$, where $R$ and $R'$ take values in $\{0,1\}^d$ representing the ``rounding direction'' of $a=\frac{\gamma_t\g f(w,S)}{\eps}$ and $a'=\frac{\gamma_t\g f(w,S_J)}{\eps}$, respectively. For example, if $\round(a_i) >= a_i$ then $R_i = 1$ otherwise $R_i=0$. Again by chain rule of KL, we have
\begin{align*}
\KL{X}{X'}\leq \KL{R}{R'} + \E_{r\in\{0,1\}^d}[\KL{X|R=r}{X'|R'=r}]
\end{align*}
Since both $R=(R_1,..,R_d)$ and $R=(R'_1,...,R'_d)$ are $d$ independent fair coins, their probability distributions should be equal. Thus $\KL{R}{R'} = 0$. Moreover, for any fixed $r\in\{0,1\}^d$, we have $X|R=r$ is a point mass on 
\[w - \lfloor a \rfloor + \eps\cdot r.\]
Therefore,
\begin{align*}
\KL{X|R=r}{X|R'=r} &= 1 \cdot \log\left(\frac{1}{\Pr[\xi_t=a]}\right)
\end{align*}
\end{proof}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the conclusion section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} It can be found in our supplemental material. 
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We only use the standard MNIST and CIFAR10 datasets.} 
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> gld_grad_con.tex <==
The following Lemma~\ref{lem:gld-grad-con} indicates that the summation in the above bound is $O(T/n)$ with high probability.

\begin{lemma}\label{lem:gld-grad-con} Suppose the loss function $f$ is $L$-Lipschitz. Let $S \in \Z^n$ be any fixed training set, and $W=(W_0,...,W_T)$ be any random sequence independent of $J$. We have the following inequality holds w.p. $\geq 1-\delta$ over the randomness of $J\sim Uniform([n])^m$:
\[\E_W\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2\right] \leq \frac{C_{\delta}}{m}\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}L^2,\]
where $C_{\delta} = 4+ 2\ln(1/\delta) + 5.66\sqrt{\ln(1/\delta)}$.
\end{lemma}
\begin{proof}
Define function $\Phi:[n]^m \to \R^+$ as follows:
\begin{align*}
    \Phi(J) := \sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2}.
\end{align*}
Let $J$ and $J'$ be any two ``neighboring'' index-sets \footnote{Formally, they should satisfy $|\{i : J_i \neq J'_i\}| = 1$.}. 
Define $A_t = \g f(W_{t-1},S) - \g f(W_{t-1}, S_J)$ and $B_t = \g f(W_{t-1},S_J) - \g f(W_{t-1},S_{J'})$. We have:
\begin{align*}
    \Phi(J')^2 &:=\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{A_t + B_t}^2\\
    &= \E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}(A_t^{\top}A_t + B_t^{\top}B_t) + 2\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}A_t^{\top}B_t\\
    &\leq \E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}(A_t^{\top}A_t + B_t^{\top}B_t) + 2\sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}A_t^{\top}A_t}\sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}B_t^{\top}B_t}\\
    &=\left(\sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{A_t}^2} + \sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{B_t}^2}\right)^2\\
    &\leq \left(\Phi(J) + \frac{2L}{m}\sqrt{\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}}\right)^2.
\end{align*}
It implies $\Phi(J') \leq \Phi(J) + \frac{2L}{m}\sqrt{\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}}$. Similarly, we can prove $\Phi(J) \leq \Phi(J') + \frac{2L}{m}\sqrt{\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}}$. Thus we have for any $J,J'$ differing in one element:
\[|\Phi(J) - \Phi(J')| \leq \frac{2L}{m}\sqrt{\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}}.\]
Applying McDiarmid's inequality, we have for any $\epsilon > 0$:
\begin{align*}
\Pr_J\left[\Phi(J) - \E_{J}[\Phi(J)] \geq \epsilon \right] \leq \exp\left(\frac{-2m\epsilon^2}{4L^2\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}}\right).
\end{align*}
We can use it to control the square of $\Phi(J)$:
\begin{align}\label{eq:gld-mcd}
    \Pr_J\left[\Phi(J)^2 \geq (\epsilon + \E_{J}[\Phi(J)])^2\right] 
    &= \Pr_J\left[\Phi(J) - \E_{J}[\Phi(J)] \geq \epsilon \right]\notag\\
    &\leq \exp\left(\frac{-2m\epsilon^2}{4L^2\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}}\right).
\end{align}
It remains to control the expectation:
\begin{align*}
\E_{J}[\Phi(J)] &= \E_{J}\sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2}\\
&\leq \sqrt{\E_W\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\E_{J}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2}\\
&\leq \sqrt{\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\frac{4L^2}{m}}.
\end{align*}
Plugging the above inequality into \eqref{eq:gld-mcd} and replacing $\epsilon$ with $\sqrt{\frac{\ln(1/\delta)4L^2\sum_{t=1}^T\gamma_t^2/\sigma_t^2}{2m}}$, we conclude that:
\begin{align*}
\Pr_J\left[\Phi(J)^2 \leq \frac{4+ 2\ln(1/\delta) + 5.66\sqrt{\ln(1/\delta)}}{m}\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}L^2\right] \geq   1-\delta.
\end{align*}
\end{proof}

Now we are ready to prove our Theorem~\ref{thm:gld-bound}, which is a direct consequence of Lemma~\ref{lem:gld-grad-con} and Corollary~\ref{cor:gld-data}.
\begin{theorem}\label{thm:gld-bound}
Let $Q_S$ be the distribution of \ref{eq:gld}'s output when training set is $S$. For any $\delta \in (0, 1)$ and $m\geq 1$, we have w.p. $\geq 1-2\delta$ over $S\sim \D^n$ and $J \sim Uniform([n])^m$, the following holds:
\begin{align*}
\loss(Q_S,\D) \leq 5.1 \loss(Q_S,S_I) &+  \frac{1.01\ln(1/\delta)}{n-m} + \frac{0.505C_{\delta}L^2}{(n-m)m}\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2},
\end{align*}
where $C_{\delta} = 4+ 2\ln(1/\delta) + 5.66\sqrt{\ln(1/\delta)}$, and $I = \{i \in [n] \,\,|\, i \notin J\}$ is the indices that are not in $J$.
\end{theorem}
\begin{proof}
Plugging Lemma~\ref{lem:gld-grad-con} into Corollary~\ref{cor:gld-data} and applying union bound, we can prove the theorem.
\end{proof}

==> old_vec_con.tex <==
The following Lemma~\ref{lem:fix-w-concentration} gives the concentration for fixed $S$ and $W$.

\begin{lemma}~\label{lem:fix-w-concentration}
For any fixed $S$ and $W=(W_0,...,W_T)$, we have:
\begin{align*}
\Pr_{J\sim Uniform([n])^m}\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2 \geq \epsilon \right] \leq 2Td \exp(-\frac{\epsilon m}{6.3L^2}),
\end{align*}
where $L = L_0\sqrt{\sum_{t=1}^T\gamma_t^2/\sigma_t^2}$ and $L_0:=\sup_{w,z} \g f(w,z)$ is the global lipschitz constant.
\end{lemma}
\begin{proof}
The sum of the squared gradient norm can be viewed as the $\ell_2$ distance of two $T \cdot d$ dimensional vectors. Formally, define $G_i \in \R^{T\cdot d}$ as follows: the element in index $(t-1)\cdot d + j$ is equal to $\frac{\gamma_t^2}{\sigma_t^2} \g_j f(W_{t-1},z_i)$. Thus we have
\[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2 = \norm{\frac{1}{m}\sum_{k=1}^m G_{J_k} - \mu}^2,\]
where $\mu := \frac{1}{n}\sum_{i=1}^n G_i = \E_{J_k \sim Uniform([n])}[G_{J_k}]$. For a fixed $k\in [m]$. Since $\norm{G_i} \leq L_0\sqrt{\sum_{t=1}^{T}\frac{\gamma_t^2}{\sigma_t^2}}=:L$ for any $i\in [n]$, the random vector $G_{J_k}$ is $cL$-norm-subGaussian (see Lemma~1 in \citet{jin2019short}). Or equivalently, for any $k\in[m]$,
\begin{align*}
    \Pr[\norm{G_{J_k} - \mu} \geq \epsilon] \leq 2e^{-\frac{\epsilon^2}{2c^2L^2}}.
\end{align*}
It directly implies $\frac{1}{m}G_{J_k}$ is $\frac{cL}{m}$-norm-subGaussian. The constant $c$ is equal to $\sqrt{2/\ln(2)}$ which is less than $1.7$. Moreover, the Hoeffding-type inequality for norm-subGaussian (Corollary 7 in \citet{jin2019short}) gives that w.p. at least $1-\delta$:
\begin{align*}
    \norm{\frac{1}{m}\sum_{k=1}^m G_{J_k} - \mu} \leq \frac{2.5L}{\sqrt{m}} \sqrt{\log\frac{2Td}{\delta}}.
\end{align*}
Thus we have for any $\delta \in (0,1)$:
\begin{align*}
\Pr_{J}\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2 \geq \frac{6.3L^2\log(2Td/\delta)}{m}\right] \leq \delta,
\end{align*}
which is equivalent to
\begin{align*}
\Pr_{J}\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2 \geq \epsilon \right] \leq 2Td \exp(-\frac{\epsilon m}{6.3L^2}).
\end{align*}
\end{proof}
The following lemma can realize the transformation of the two definitions of subGaussian.
\begin{lemma} \label{lem:prob-Eexp}
Suppose $A > 0$ is a random variable s.t. $\Pr[A \geq \epsilon] \leq 2K \exp(-\epsilon)$, then $\E[e^{A/5}] \leq 8K$.
On the other hand, if $\E[e^A] \leq 2K$, then $\Pr[A \geq \epsilon] \leq 2K e^{-\epsilon}$.
\end{lemma}
Combing Lemma~\ref{lem:fix-w-concentration} and Lemma~\ref{lem:prob-Eexp}, we have the following corollary.
\begin{corollary}\label{cor:KL-bound}
For any fixed $S$, we have w.p. at least $1-\delta$ over $J\sim Uniform([n])^m$:
\begin{align*}
\E_{W}\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2\right] \leq \frac{ 31.5\ln(8Td/\delta)L_0^2\sum_{t=1}^T\gamma_t^2/\sigma_t^2}{m},
\end{align*}
where $L_0:=\sup_{w,z} \g f(w,z)$ is the global lipschitz constant and $W$ is the training trajectory of SGLD when input is $S$.
\end{corollary}
\begin{proof}
Let $B(W) = \sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2$ be the cumulative squared gradient norm for a given $W$. Let $A(W)$ be $\frac{m}{6.3L^2}B(W)$. Applying Lemma~\ref{lem:fix-w-concentration} we have for any fixed $W$:
\begin{align*}
    \Pr_{J}[A(W) \geq \epsilon] \leq 2Tde^{-\epsilon}.
\end{align*}
Then plugging it into Lemma~\ref{lem:prob-Eexp} with $K=Td$, we have
\begin{align*}
\E[e^{A(W)/5}] \leq 8Td.
\end{align*}
By Jensen's inequality and convexity of exp function, we have 
\begin{align*}
\E_J\left[\exp(\E_{W}[A(W)/5])\right] &\leq \E_W\E_J\left[\exp(A(W)/5)\right]\\
&\leq 8Td.
\end{align*}
By the second part of Lemma~\ref{lem:prob-Eexp}, we have
\[\Pr\left[\E_{W}[A(W)/5] \geq \epsilon \right] \leq 8Td e^{-\epsilon}.\]
Plugging the definition of $A(W)$ into the above inequality, we have
\begin{align*}
\Pr_J\left[\frac{m}{6.3L^2}\E_{W}\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2\right] \geq 5\epsilon \right] \leq 8Td e^{-\epsilon}.
\end{align*}
Let $\delta = 8Tde^{-\epsilon}$, we can rewrite the above inequality to
\begin{align*}
\Pr_J\left[\E_{W}\left[\sum_{t=1}^T\frac{\gamma_t^2}{\sigma_t^2}\norm{\g f(W_{t-1},S) - \g f(W_{t-1},S_J)}^2\right] \geq \frac{\ln(8Td/\delta) \cdot 5 \cdot 6.3L_0^2\sum_{t=1}^T\gamma_t^2/\sigma_t^2}{m} \right] \leq \delta.
\end{align*}
\end{proof}
Directly combining Corollary~\ref{cor:KL-bound} and Corollary~\ref{cor:sgld-data}, and using union bound, we have the following generalization bound for SGLD.
\begin{theorem}
For any $\delta \in (0, 1)$ and $m\geq 1$, we have w.p. at least $1-2\delta$ over $S\sim \D^n$ and $J \sim Uniform([n])^m$, the following holds:
\begin{align*}
\loss(Q,\D) \leq 5.1 \loss(Q,S_I) +  \frac{1.01\ln(1/\delta)}{n-m} + \frac{16\ln(8Td/\delta)L_0^2\sum_{t=1}^T\gamma_t^2/\sigma_t^2}{(n-m)m},
\end{align*}
where $I = \{i\in[n]\,\,|\,\,i \notin J\}$, $d$ is the dimension of the parameter and $L_0:=\sup_{w,z} \g f(w,z)$ is the global lipschitz constant.
\end{theorem}
